GhostEncoder: Stealthy Backdoor Attacks with Dynamic Triggers to Pre-trained Encoders in Self-supervised Learning

Within the realm of computer vision, self-supervised learning (SSL) pertains to training pre-trained image encoders utilizing a substantial quantity of unlabeled images. Pre-trained image encoders can serve as feature extractors, facilitating the construction of downstream classifiers for various tasks. However, the use of SSL has led to an increase in security research related to various backdoor attacks. Currently, the trigger patterns used in backdoor attacks on SSL are mostly visible or static (sample-agnostic), making backdoors less covert and significantly affecting the attack performance. In this work, we propose GhostEncoder, the first dynamic invisible backdoor attack on SSL. Unlike existing backdoor attacks on SSL, which use visible or static trigger patterns, GhostEncoder utilizes image steganography techniques to encode hidden information into benign images and generate backdoor samples. We then fine-tune the pre-trained image encoder on a manipulation dataset to inject the backdoor, enabling downstream classifiers built upon the backdoored encoder to inherit the backdoor behavior for target downstream tasks. We evaluate GhostEncoder on three downstream tasks and results demonstrate that GhostEncoder provides practical stealthiness on images and deceives the victim model with a high attack success rate without compromising its utility. Furthermore, GhostEncoder withstands state-of-the-art defenses, including STRIP, STRIP-Cl, and SSL-Cleanse.

==> header/header-Tikz.tex <==

\usetikzlibrary{arrows,positioning, shapes, calc, backgrounds, fit, shadows}
\usetikzlibrary{matrix,shapes,arrows,positioning,chains,calc}
\usetikzlibrary[shapes.arrows]
\usetikzlibrary{shapes.geometric}
\usetikzlibrary{arrows}
\usetikzlibrary{backgrounds}
\usetikzlibrary{matrix}
\usetikzlibrary{positioning}
\usetikzlibrary{calc}
\usetikzlibrary{intersections}
\usetikzlibrary{fadings}
\usetikzlibrary{decorations.footprints}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{patterns}
\usetikzlibrary{shapes.callouts}
\usetikzlibrary{fit}
%%% TIKZ/PGF COMMANDS
\usetikzlibrary{matrix}
\usetikzlibrary{calc}
\usetikzlibrary{shadows}
\usetikzlibrary{scopes}
\usetikzlibrary{chains}
\usetikzlibrary{positioning}
\usetikzlibrary{fit}
\usetikzlibrary{backgrounds}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{shapes.geometric}
\usetikzlibrary{shapes.symbols}
\usetikzlibrary{shapes.misc}
%%% By Zengpeng Li
\usetikzlibrary{arrows}
% color aliases
%\colorlet{Lattice}{Green}
%\colorlet{Set}{Red!10}

% global styles
\tikzset{
  % make drop shadows a bit softer
  every shadow/.style={opacity=.4,shadow xshift=.3ex,shadow yshift=-.3ex},
  % use \& to separate cells in matrices, avoiding fragility in beamer frames
  every matrix/.style={ampersand replacement=\&},
  % edges and joins with arrows and thicker
  every edge/.append style={->,thick},
  every join/.style={->,thick},
  % distance between nodes
  % node distance=1ex and 2ex,
}

% styles for drawing in Rn, especially lattices
\tikzset{
  % lattice transform must include "cm" dimension to work properly,
  % otherwise the x and y transforms become dependent
  Ztrans/.style={x={(1.5cm,1cm)},y={(.5cm,1.5cm)}},
  Zdual/.style={x={(1.5cm,-.5cm)},y={(.5cm,1cm)}},
  latttrans/.style={x={(1.8cm,.5cm)},y={(0.4cm,1.3cm)}},
  dualtrans/.style={x={(1.3cm,-.4cm)},y={(-.5cm,1.8cm)}},
  lattB/.style={x={(1.8cm,.5cm)},y={(0.4cm,1.4cm)}},
  dualB/.style={x={(1.4cm,-.4cm)},y={(-.5cm,1.8cm)}},
  shortB/.style={x={(.5cm,.2cm)},y={(-.1cm,1.7cm)}},
  latt2B/.style={x={(1cm,.1cm)},y={(.1cm,1.2cm)}},
  ulattB/.style={x={(2.0cm,.5cm)},y={(2.1cm,-.2cm)}},
  openball/.style={fill=Blue!20},
  ball/.style={openball,thin,draw=Blue},
  latt/.style={Lattice,fill},
  dist/.style={Brown,densely dashed,font=\footnotesize},
  offlabel/.style={Brown,inner sep=2pt,font=\footnotesize},
  axes/.style={->,Gray,style=very thin},
  fundamental/.style={Gray,fill opacity=.2},
  target/.style={fill,Brown},
  project/.style={thin,dashed},
  help lines/.style={Gray,very thin,step=.5cm},
  % expanding waves representing noise
  noise/.style={
    Lattice,
    opacity=.5,
    decorate,decoration={
      expanding waves,
      segment length=5pt,angle=10,
      post=moveto,post length=3pt
    },
  },
}

% lattice that can be dropped into any path.
% it would be sensible to set a default argument here, but
% commands with optional args don't parse correctly inside a
% tikz path
\newcommand*{\latt}[1]{%
  \foreach \a in {-4, ..., 4} {
    \foreach \b in {-4, ..., 4} {
      (\a,\b) circle (#1)
    }
  }
}


%%% COMMANDS FOR LECTURES/HOMEWORKS









%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
%Draw brace
%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
\tikzset{
    ncbar angle/.initial=90,
    ncbar/.style={
        to path=(\tikztostart)
        -- ($(\tikztostart)!#1!\pgfkeysvalueof{/tikz/ncbar angle}:(\tikztotarget)$)
        -- ($(\tikztotarget)!($(\tikztostart)!#1!\pgfkeysvalueof{/tikz/ncbar angle}:(\tikztotarget)$)!\pgfkeysvalueof{/tikz/ncbar angle}:(\tikztostart)$)
        -- (\tikztotarget)
    },
    ncbar/.default=0.5cm,
}

\tikzset{square left brace/.style={ncbar=0.5cm}}
\tikzset{square right brace/.style={ncbar=-0.5cm}}

\tikzset{round left paren/.style={ncbar=0.5cm,out=120,in=-120}}
\tikzset{round right paren/.style={ncbar=0.5cm,out=60,in=-60}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% for double arrows a la chef
% adapt line thickness and line width, if needed
\tikzstyle{vecArrow} = [thick, decoration={markings,mark=at position
   1 with {\arrow[semithick]{open triangle 60}}},
   double distance=1.4pt, shorten >= 5.5pt,
   preaction = {decorate},
   postaction = {draw,line width=1.4pt, white,shorten >= 4.5pt}]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Draw Alice and Bob
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usetikzlibrary{calc,shapes.callouts}
\newcommand{\calloutquote}[3][.95\textwidth]{%
    \setbox0=\vbox{\parbox[b]{#1}{#3}}
    \setlength{\calloutheight}{\ht0+\calloutoffset}
    \setlength{\quoteheight}{\calloutheight+2\baselineskip}
    \par\vspace*{\quoteheight}
    \noindent\hfil
  \tikz[remember picture]{
        \node [anchor=base,inner sep=0,outer sep=0,
        text width=#1,align=center] (#2) {#2};
    \node[anchor=base,overlay,rectangle callout,
        callout relative pointer={(-0.3cm,-0.7cm)},
        fill=blue!30,text width=#1,align=justify]
        at ($(#2.north)+(0,\calloutheight)$) {#3};}
}


\definecolor{gauss}{rgb}{0.8,0.2,0.2}
\definecolor{RegionColor}{rgb}{0.89,0.89,0.58}
\definecolor{Math}{rgb}{0.05,0.05,0.55}
\definecolor{Curva}{rgb}{0.10,0.20,0.30}
\definecolor{FillBox}{rgb}{1,0.8,0.2}
\definecolor{Facts}{rgb}{0.05,0.95,0.05}
\definecolor{Sign}{rgb}{0.7,0.95,0.7}
\definecolor{Ver}{rgb}{0.7,0.95,0.2}
\definecolor{pink}{rgb}{1,0.75,0.80}
\definecolor{v1}{rgb}{1,0.4,0.2}
\definecolor{v2}{rgb}{0.2,0.4,1}
\definecolor{pc}{rgb}{0.94,0.98,0.75}


\tikzstyle{Box}=[rectangle,draw=Curva,fill=FillBox,rounded corners, minimum width=1.3cm]
\tikzstyle{aBox}=[rectangle,draw=black,rounded corners, yshift=0.5cm]
\tikzstyle{acBox}=[rectangle,draw=black, fill=Sign, rounded corners, yshift=0.5cm, text width=1.3cm, align=center]
\tikzstyle{lBox}=[rectangle,draw=Curva,fill=FillBox,rounded corners, minimum width=1.3cm]
\tikzstyle{fBox}=[rectangle,draw=black, fill=Facts,rounded corners, minimum width=3cm]
\tikzstyle{lmBox}=[rectangle,draw=Curva,fill=FillBox,rounded corners] % Zpli
\tikzstyle{mBox}=[rectangle,draw=black,rounded corners]
\tikzstyle{sBox}=[rectangle,draw=black]
\tikzstyle{pBox}=[rectangle,draw=black, fill=pc]
\tikzstyle{rBox}=[rectangle,draw=black, fill=red!95,rounded corners]
\tikzstyle{gBox}=[rectangle,draw=black, fill=green!75,rounded corners]
\tikzstyle{bBox}=[rectangle,draw=black, fill=blue!25,rounded corners]
\tikzstyle{Circ}=[circle,draw=black, fill=RegionColor!75]








==> header/header-protocol.tex <==
% !TEX root = mainCMDVNIZK.tex

%%%%%%%%%%%%%%
%nice figure
%%%%%%%%%%%%%%
\newcommand{\mybox}[5]{
    \begin{figure*}[tp]
        \centering
    \begin{tikzpicture}
        \node[anchor=text,text width=\columnwidth-1.0cm, draw, rounded corners, line width=1pt, fill=#3, inner sep=2mm] (big) {\\#4};
        \node[draw, rounded corners, line width=.5pt, fill=#2, anchor=west, xshift=5mm] (small) at (big.north west) {#1};
    \end{tikzpicture}
    \caption{#5}
    \end{figure*}
    \vspace{-2mm}
}




\newenvironment{nfprot}[1]{%
  \footnotesize
  \begin{mdframed}
    \begin{minipage}{\linewidth}
      {\begin{center}\underline{\textbf{Protocol} #1}\end{center}}
}{%
    \end{minipage}
  \end{mdframed}
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newlength{\protowidth}
\newcommand{\pprotocol}[5]{
{\begin{figure*}[#4]
\begin{center}
\setlength{\protowidth}{\textwidth}
\fbox{
        \small
        \hbox{\quad
        \begin{minipage}{\protowidth}
    \begin{center}
    {\bf #1}
    \end{center}
        {\fontsize{8pt}{9pt} \selectfont #5}
        \end{minipage}
        \quad}
        }
        \caption{\label{#3} #2}
\end{center}
\vspace{-4ex}
\end{figure*}
} }




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\newcommand{\pprotocolbest}[6]{
	{\begin{figure*}[#4]
			\begin{center}
				\setlength{\protowidth}{.9\textwidth}
				\fbox{
					\small
					\hbox{\quad
						\begin{minipage}{\protowidth}
							\begin{center}
								{\bf #1}
							\end{center}
							#6
						\end{minipage}
						\quad}
				}		
			\end{center}
			\caption{\label{#3} #2}
			{\small 	#5		}
			
			
		\end{figure*}
	} }




%%% import zli
\newcounter{protocol}
\newenvironment{xprotocol}[1]
  {\par\addvspace{\topsep}
   \noindent
   \tabularx{\linewidth}{@{} X @{}}
    \hline
    \refstepcounter{protocol}\textbf{Protocol \theprotocol} #1 \\
    \hline}
  { \\
    \hline
   \endtabularx
   \par\addvspace{\topsep}}

\newcommand{\sbline}{\\[.1\normalbaselineskip]}% small blank line




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newenvironment{code}[2]{
  \small
  \begin{center}
    \fbox{\parbox{#1\textwidth}{%
        \vspace{-13pt}
        \begin{tabular}{l}
          \hspace{-7pt}
          \parbox[t]{\textwidth}{%
          #2
          }
        \end{tabular}
        \vspace{-3ex}
      }
    }
}{%
  \end{center}
  \vspace{-3ex}
}

\newenvironment{codetwo}[3]{%
  \small
  \begin{center}
    \begin{tabular}{l}
      \fbox{\parbox[t]{#1\textwidth}{%
      #2
      }}
      \\
      \fbox{\parbox[t]{#1\textwidth}{%
      #3
      }}
}{%
    \end{tabular}
    \vspace{-3ex}
  \end{center}
}

\newenvironment{codethree}[4]{%
  \small
  \begin{center}
    \begin{tabular}{l}
      \fbox{\parbox[t]{#1\textwidth}{%
      #2
      }}
      \\
      \fbox{\parbox[t]{#1\textwidth}{%
      #3
      }}
      \\
      \fbox{\parbox[t]{#1\textwidth}{%
      #4
      }}
}{%
    \end{tabular}
    \vspace{-3ex}
  \end{center}
}




